Creativity in Machine Learning

Recent machine learning techniques can be modified to produce creative results. Those results did not exist before; it is not a trivial combination of the data which was fed into the machine learning system. The obtained results come in multiple forms: As images, as text and as audio. This paper gives a high level overview of how they are created and gives some examples. It is meant to be a summary of the current work and give people who are new to machine learning some starting points.

==> Makefile <==
SOURCE = art-in-machine-learning
make:
	pdflatex -shell-escape $(SOURCE).tex -interaction=batchmode -output-format=pdf # aux-files for makeindex / makeglossaries
	makeglossaries $(SOURCE)
	bibtex $(SOURCE)
	pdflatex -shell-escape $(SOURCE).tex -interaction=batchmode -output-format=pdf # include index
	pdflatex -shell-escape $(SOURCE).tex -interaction=batchmode -output-format=pdf # include symbol table
	pdflatex -shell-escape $(SOURCE).tex -interaction=batchmode -output-format=pdf # include symbol table
	make clean

arxiv:
	rm upload.zip
	make clean
	zip -r upload.zip . -x \*.git\* -x MAKEFILE -x *.zip -x *.pdf -x *.md -x *.sublime\* -x vortrag\* -x presentation-images\* -x figures/eth-faces\* -x figures/DeepDream/Sky\* -x figures/DeepDream/plant\*

clean:
	rm -rf $(TARGET) *.class *.html *.aux *.out *.thm *.idx *.toc *.ilg *.glg *.glo *.gls *.ist *.xdy *.fdb_latexmk *.bak *.blg *.glsdefs *.acn *.acr *.alg *.nls *.nlo *.bak *.pyg *.lot *.lof *.xmpdata *.xmpi *.bak
	# rm -rf *.bbl *.ind  # Needed for arxiv
	rm -rf *.log   # Needed for checking
